CBR-iKB: A Case-Based Reasoning Approach for Question Answering over Incomplete Knowledge Bases

Knowledge bases (KBs) are often incomplete and constantly changing in practice. Yet, in many question answering applications coupled with knowledge bases, the sparse nature of KBs is often overlooked. To this end, we propose a case-based reasoning approach, CBR-iKB, for knowledge base question answering (KBQA) with incomplete-KB as our main focus. Our method ensembles decisions from multiple reasoning chains with a novel nonparametric reasoning algorithm. By design, CBR-iKB can seamlessly adapt to changes in KBs without any task-specific training or fine-tuning. Our method achieves 100% accuracy on MetaQA and establishes new state-of-the-art on multiple benchmarks. For instance, CBR-iKB achieves an accuracy of 70% on WebQSP under the incomplete-KB setting, outperforming the existing state-of-the-art method by 22.3%.

==> commented_introduction.tex <==
% Para1: straight intro to the task. KBs are woefully incomplete (Min et al. 2013). We consider a realistic setting for KBQA where the given KB is sparse. ALso try to mention how much information is present in text (and not in KB because KB building is hard) and we need methods which can seamlessly use both.
% Para2: Next, make this point clear bringing the paragraph starting line 98.
% Para3: Introduce CBR. Start by saying, that you dont have annotated reasoning patterns (logical forms), i.e. weakly supervised. Often the reasoning patterns used for answering a similar question are same for a given question. Refer to figure and show that the reasoning paths are indeed same. Then say CBR is a grand symbolic AI methodology and briefly describe 4 steps (feel free to adapt text from paragraph 1 of EMNLP paper). May be at the end of the para, you can say Das, Thai et al 2021 does CBR they use strong supervision which has a lot of limitations.

%Para4: You get a simialr question by comparing pre-trained LM representations from the training set. The you obtain reasoning patterns. You also should mention how you get text. And then how reasoning patterns dont execute (refer to figure 2), and then you use beam search and text. But sometimes text fails and then we use KBC (again refer to figure 2)

% Para5. 2 lines about how you get great results

%Para 6. List of contributions.

% Various approach for knowledge base question answering (KBQA) has been developed (cite your favorite 5 papers) and significantly improved the state-of-the-art on KBQA tasks. 
% However, most of the work operate with the assumption that the given underlying KB has sufficient evidence to answer the questions. 
% For example, MINERVA, Transfernet operate directly on the KB by finding chains of relations that connect the question entities to the answer. However, in practice KBs can be woefully incomplete (\cite{min2013}), missing a lot of intermediate relations making the actual problem much more challenging.
% There has been some recent work which are designed to work on the more realistic setting of incomplete KGs (\cite{Stanford, EmbedKGQA}). For example, EmbedKGQA achieves this by randomly dropping up to 50% of edges in the KG. In practice, only 15.75\% (train), 14\% (dev), and 15.34\% (test) questions are affected.
% Why would a CBR like model help the incomplete setting?

% Knowledge base question answering (KBQA) task aims to solve natural language queries with background knowledge stored in a knowledge base.
% Knowledge bases (KB) consist of real-world entities and their relationships in the form of triples, such as \texttt{(J.K.Rowling, birthplace, United Kingdom)}.
% Over the years, advancing knowledge-base question answering systems continuously attracts research attention from both academia and industry.
% I want to give a 1-liner survey to KBQA methods here. So I still think that we should properly cite the literature.
% Various approaches have been developed from rule-based systems [?], knowledge graph embeddings~\citep{saxena2020embedkgqa}, reinforcement learning~\citep{das2018minerva}, graph query generation~\citep{shi2021transfernet}, neural semantic parsing~\citep{cai2013largescaleSP, chen2021retrack} have been developed and significantly improved state-of-the-art KBQA performances.

% However, the high-performance regime of KBQA systems is often tied with supervised learning and with an ideal, complete knowledge base provided.
% In practice, the annotation cost for supervised KBQA is high, and knowledge base are woefully incomplete~\citep{min2013distant}.
% There are some recent works~\citep{sun2018graftnet,sun2019pullnet, saxena2020embedkgqa,sun2020faithful,ren2021lego,shi2021transfernet} which are designed to work on incomplete knowledge bases, with only question-answer pairs available at training time (weakly-supervised).
% They show that KBQA performances on incomplete KB can be improved with text and knowledge base embeddings. 
% Nevertheless, there are still strong gaps in performance when KB relations are missing.

==> conclusion.tex <==
\section{Conclusions}
We proposed \method - a nonparametric, instance-based method for question answering over knowledge base.
Our method performs well on multiple benchmarks [?], given only weak-supervision learning signals.
It achieved 100\% accuracy on the MetaQA dataset.
On WebQuestionSP, our method outperforms other state-of-the-art models significantly for question answering over incomplete knowledge base. 
The qualitative analysis demonstrates that \method's predictions are interpretable and explainable.
Such features are shown to be useful in practice, and can further improve WebQuestionSP results by xx\%.

Our proposed KBQA system also has a major drawback. 
It works based on the assumption that solutions to a question are previously seen for some similar questions.
Therefore our method are not able to generalize to novel compositional questions.
Nevertheless, it works well for KBQA tasks where similar questions are frequently asked.
There are some interesting research directions to enable compositional QA for our method.
Question decomposition can be used to simplify input questions.
The casebase can also be improved by adding questions from generation models.

==> experiments.tex <==

\section{Experiments}

In this section, we evaluate \sysname against 4 baselines on 2 datasets across complete and incomplete KB settings. We validate the following claims: (a) \textcolor{red}{Claim 1}  (b) \textcolor{red}{Claim 2} 

\subsection{Datasets}
We evaluate our model on two datasets: MetaQA \cite{zhang2018variational} and WebQuestionSP \cite{yih2016value}, described in Table \ref{tab:dataset}.
% These two datasets were created under the assumption that the correct inferential chains exist in the knowledge base, i.e., the KB is complete for the given QA pairs.


\begin{table}[]
    \centering
    \begin{tabular}{l|ccc}
        \hline \textbf{Dataset} & \textbf{Train} & \textbf{Dev} & \textbf{Test} \\
        \hline MetaQA 1-hop & 96,106 & 9,992 & 9,947 \\
        MetaQA 2-hop & 118,948 & 14,872 & 14,872 \\
        MetaQA 3-hop & 114,196 & 14,274 & 14,274 \\
        \hline WebQuestionSP & 2,848 & 250 & 1,639 \\
        % \hline CompWebQ & 27,623 & 3,518 & 3,531 \\
        \hline
    \end{tabular}
    \caption{Dataset statistics.}
    \label{tab:dataset}
\end{table}


\paragraph{MetaQA} \cite{zhang2018variational} is a multi-hop QA dataset with approximately 400K questions, that extends the WikiMovies dataset [?] beyond 1-hop to 2-hop and 3-hop questions. 
The questions are generated from twelve templates.
% , such as ``Who starred in the movies directed by X’’.
The KB contains 43K entities and 8 relations from the movie domain, with 135K triples in total. 
Questions in MetaQA are answerable using the corpus ($\sim 18K$ passages) provided in the original WikiMovies dataset. 

\textcolor{red}{What does this mean?} - We follow \textcolor{red}{CITE} and use exact match of surface forms to extract entity mentions and link them to the KB for both questions and documents in the text corpus.
We later show in Section \ref{sec:appendix} that the KB reinforced with text in such way leaves out useful information in text. 
To better utilize the text corpus, we suggest using a coreference model [?] and demonstrate that co-referenced entities can compensate a significant number of missing relations in the KB. 

While \textcolor{red}{CITE} uses exact match of surface forms to extract entity mentions and link them to the KB for both questions and documents in the text corpus, we show in Section \ref{sec:appendix} that this is suboptimal and disregards valuable information in the text.
We instead demonstrate that the use of a co-reference model improves the relevancy of linked text and improves QA performance.


\paragraph{WebQuestionsSP} [?] is a real-world question answering dataset using Freebase as its knowledge base.
It is a subset of the WebQuestions [?] dataset whose questions are crawled from Google Suggest API and answers are obtained from Amazon Mechanical Turk.
The WebQuestionSP dataset has 4887 questions, each question is coupled a topic entity, a gold inferential chain, and set of additional constraints.
Its questions are either 1-hop or 2-hop.
Similar to [?] we use the triples within 2-hop from entities mentioned in the target question as its target sub-KB.
As for the text corpus, we use the set of Wikipedia documents provided by GRAFT-Nets [?].
For each question, GRAFT-Nets retrieves the top 50-sentences that are relevant to mentioned entities.

In both these datasets, the complete inferential chain required to answer each question is present in the KB.
% To evaluate QA systems in an incomplete-KB setting, we follow \cite{embedkgqa} and drop triples from the KB to simulate missing edges.
% For WebQuestionSP, we found that the majority of dropped triples used in \citep{embedkgqa} do not directly affect QA performance.
To simulate an incomplete-KB setting, prior work \textcolor{red}{CITE} has randomly dropped some fraction of the triples in the KB. However, we find that the fraction of actual questions in these datasets affected when dropping half the KB triples is much smaller (only 15\%).   
Thus the reported performances for the incomplete-KB setting involve a large number of questions that are in fact complete.
% Hence we propose a new scheme to induce incompleteness that renders at least 50\% of QA pairs having missing relations in their original inferential chains. 
Hence we propose a new scheme to induce incompleteness that provides a more accurate evaluation of performance.

\input{tab_main_results}

\subsection{Baselines}
We compare \method with three baselines: GRAFT-Net \cite{sun2018open}, EmbedKGQA \cite{embedkgqa}, and TransferNet \cite{shi2021transfernet}.

\textbf{GRAFT-Net} is a graph convolution based model that operates over a graph of KB triples and text documents.
It was one of the earliest papers that study question answering with an incomplete knowledge base.
The suite of benchmark tasks proposed in GRAFT-Net is used in both EmbedKGQA and TransferNet. 
Furthermore, GRAFT-Net provides the evaluation for the text only and combined text-KB setting for the two datasets, which other baselines lack of.
PullNet [?] is a more recent improved version of GRAFT-Net with a learned, CNN based subgraph retriver.
However, its experiments are not reproducible.
Therefore, we only report its numbers taken from [?].

\textbf{EmbedKGQA} treats question embeddings as latent relation representations and jointly trains them with KB triples.
It was the state-of-the-art model for the WebQuestionSP dataset with an incomplete KB.
In their experiments, EmbedKGQA randomly drop half of the KB triples, but the set of dropped triples only affects 15.75\%, 14\%, and 15.34\% of questions in the train/dev/test set, respectively.

{\color{red}Briefly summarize PullNet}

\textbf{TransferNet} proposes a step-wise, attention-based neural network model that simultaneously traverses the knowledge graph and its alternative text form.
It was the state-of-the-art on both datasets with the full KB, and on MetaQA with the half KB. 

For all baselines, we take their numbers reported in [?] whenever it is possible, and re-run experiments for WebQuestionSP with our proposed incomplete KB.

\subsection{Incomplete KB Evaluation}
We propose \textit{randomly dropping triples per question} to simulate a more rigorous evaluation for incomplete KBQA, especially for small scale question answering dataset with large scale knowledge base like WebQuestionSP.
In WebQuestionSP, only small portion of triples are in gold reasoning chains of the QA dataset.
Therefore randomly dropping triples from the entire KB does not guarantee that the majority of questions is affected.
Furthermore, questions in WebQuestionSP usually have multiple valid answers, and the QA system can simply provide answers with reasoning chains remain intact.
Taking everything into consideration, we suggest a triples dropping scheme that is QA-oriented in addition to randomly dropping.
For each question in the dataset, we decide whether to drop its triples with some probability $p$.
Next we randomly pick a relation from the gold inferential chain, and drop all triples in the sub-KB associated with the selected relation.
We can control the percentage of questions with incomplete KB by modifying $p$.
We apply our triples dropping scheme on WebQuestionSP with $p = 0.5$.
In addition, we still randomly drop triples from entire KB to simulate the effect of incomplete KB on knowledge base completion models.

\subsection{Implementation Details}
\textbf{Cases Retriever.} Our cases retriever consists of a question encoder and a dense-retriever.
We use FAISS [?], a standard dense-retriever for our task.
Regards the question encoder, we experimented with different pre-trained language model models [?] and empirically choose the best one [?].
We also conduct a small evaluation set of questions and their ideal k-nearest neighbors and manually check retriever results.

\noindent\textbf{Graph APIs.} Our graph traversal and handling algorithms are implemented using Graph-Tool [?]. All experiments with the proposed QA system were ran on a shared 2x Intel Xeon Silver CPU node with 1x V100 GPU.

\noindent\textbf{Knowledge Base Completion Model.} We employ the LibKGE [?] training, hyperparameters tuning and evaluation pipeline.
Due to resource constraints, we only consider the ComplEx model [?] and leave further investigations of others for future work.
We report the detailed evaluation of knowledge base completion models in Appendix [?].

\noindent\textbf{Relation Extraction Model.} In Section [?] we propose the use of a relation extraction model for aligning k-nearest neighbor relations and relations in the target question sub-KB.
We experimented with two relation extraction models: (1) a BERT-based relation ranker for MetaQA, and (2) the Wiki80-CNN model from the OpenNRE tool-kit [?] for WebQuestionSP.
Inputs to the relation extraction model are documents from the text corpus and the proxy-text for relations in the KB.
Mention spans of pairs of subject and object entity are also provided.
For (1) tokens within mention spans are replaced with the $\texttt{<MASK>}$ token.
For (2) mention spans are marked with [?] and [?].
We describe the process to acquire proxy-text for KB relations in more details in Appendix [?].

\subsection{Main Results}
Table ~\ref{tab:main_results} presents the performance of all QA systems coupled with the full-KB and the half-KB.
\method solved the MetaQA dataset, achieving 100\% accuracy for all MetaQA sub-tasks.
On WebQuestionSP dataset, our model achieves competitive performance with the state-of-the-art models, \textit{without any training or fine-tuning}.
On the WebQuestionSP dataset coupled with half-KB, we outperforms state-of-the-art models by a large margin (7.5\% absolute gain).
The experimental results demonstrate that CBR-based method can achieve competitive performances on the knowledge base question answering task, with weak-supervision, and incomplete knowledge bases.

Another major advantage of \method stems from its instance-based nature is that its predictions are fully self-explanatory. 
In Table [?], we present some example questions, showing their k-nearest neighbor questions and the best inferential chain our method picks up for reasoning.
One can look at incorrect \method predictions and learns where errors originate from, and further fixes these errors in a human-in-the-loop setting.
To demonstrate the ability of our proposed system to automatically fixing itself, we run our revise step on WebQuestionSP test set after each prediction and report the results in Table [?].
Similar to [?], we also conduct a human-in-the-loop experiment on the WebQuestionSP dataset.
In addition to gold inferential chains given for the full-KB, we manually annotate inferential chains for half-KB by selecting the best inferential chain that \method generates for examples in the casebase.
We report our method’s performance in Table [?].
The results show that \method is useful for practical settings where quick fixing of system predictions are desirable.

% \begin{table*}[t]
%   \centering
%     \begin{tabular}{l|ccc}
%     \hline Model & \multicolumn{3}{|c}{ MetaQA }\\
%     \cline { 2 - 4 } & 1-hop & 2-hop & 3-hop \\
%     \hline KVMemNN (Miller et al., 2016) & $95.8$ & $25.1$ & $10.1$\\
%     VRN (Zhang et al., 2017) & $97.5$ & $89.9$ & $62.5$\\
%     GraftNet (Sun et al., 2018) & $97.0$ & $94.8$ & $77.7$ \\
%     PullNet (Sun et al., 2019) & $97.0$ & $99.9$ & $91.4$ \\
%     % SRN (Qiu et al., 2020) & $97.0$ & $95.1$ & $75.2$ & $-$ & $-$ \\
%     % ReifKB (Cohen et al., 2020) & $96.2$ & $81.1$ & $72.3$ & $52.7$ & $-$ \\
%     EmbedKGQA (Saxena et al., 2020) & $97.5$ & $98.8$ & $94.8$ \\
%     TransferNet (Shi et al., 2021) & $97.5$ & $\mathbf{100}$ & $\mathbf{100}$  \\
%     \hline
%     CBR-iKB (Ours) & $\mathbf{100}$ & $\mathbf{100}$ & $\mathbf{100}$ \\
%     \hline
%     \end{tabular}
%   \caption{Blabla}
%   \label{tab:1}
% \end{table*}

% \begin{table*}[t]
%   \centering
%     \begin{tabular}{l|c|c}
%     \hline Model & WebQSP KG-Full & WebQSP KG-50 \\
%     \hline GraftNet & $66.4$ & $27.7$ \\
%     PullNet & $68.1$ & $-$ \\
%     EmbedKGQA & $66.6$ & $47.5$ \\
%     \hline CBR-iKB (Ours) & $\mathbf{69.6}$ & $\mathbf{55.7}$ \\
%     \hline
%     \end{tabular}
%   \caption{Blabla}
%   \label{tab:1}
% \end{table*}

\subsection{Ablation Study}
Table ~\ref{tab:ablation_meta} and Table ~\ref{tab:ablation_webq} show results of the ablation study on MetaQA and WebQuestionSP.
\td{Which component gives the biggest performance gains?}

\input{tab_ablation}

So far we observe that incorporating text into the knowledge base \textit{improves answers retrieval} [?].
However QA performance gains using text are marginal accross baselines [?].
We perform an error analysis on MetaQA and WebQuestionSP.
First we confirm whether text-relation edges enable path between query entity nodes and answering nodes.
In Table [?], we present number of questions with answers become reachable after adding text-relation edges.
\td{On MetaQA, we can see that ...}
\td{On WebQuestionSP, ...}
To further improve the reach-ability of answering nodes, we suggest adding text-relation edges with co-referenced mentions.

==> methods.tex <==
\section{Proposed Method}
Case-Based Reasoning (CBR) is an instance-based method, first introduced in [?] and recently adapted for supervised KBQA in [?].
In a CBR system, train samples (or \textbf{cases}) are kept in a case-base.
When a new question (or \textbf{target case}) arrives, the CBR system searches the case-base for similar questions (or the \textbf{k-nearest neighbor cases}) and their inferential chains (or \textbf{solutions}).
It then reuses retrieved solutions to predict inferential chains, executes them by traversing the knowledge base, and yields desired answers.
However, the retrieved solutions are not guaranteed to be  correct and globally consistent.
Therefore, the CBR system follows up with a revise step and a retain step that refines solutions in the case-base.
In our work, the revise step computes a ranking over the solutions.
Based on this ranking, our retain step discards solutions and cases that are likely spurious.
An illustration of our proposed pipeline, \method{}, {\color{red}is shown in Figure [?]}.

\subsection{The Case-base}
A CBR system operates on a case-base of previously seen samples and their solutions.
This section formally defines our case-base and describes how we construct it from the training dataset.

A case-base $\mathcal{C}$ is a set of cases, where each case $c$ is a pair of (1) a case representation $\mathbf{x}$, and (2) a set of inferential chains $\mathcal{P}$. 
Given the knowledge base $K$ and a pre-trained language model $\texttt{LM}$, we can formally define $c$ as follows.
\begin{align*}
    c \coloneqq (\mathbf{x}, \mathcal{P}) \coloneqq \big(\texttt{LM}(q_{\texttt{<MASK>}}), \{\mathbf{p} \mid K, \mathcal{E}_q, \mathcal{E}_a \}\big)
\end{align*}
where $q, \mathbf{p}, \mathcal{E}_q, \mathcal{E}_a$ are the question,  the corresponding inferential chain, the answer set, and the set of extracted query entities from $q$.

Now, we describe how we use each question-answers sample $(q, \mathcal{E}_a)$ from the training dataset to derive a case in the case-base. 
First, we use pre-trained language model $\texttt{LM}$ to encode the question $q$ and produce a case representation $\mathbf{x}$, similar to [?].
By the similarity definition in Section~\ref{}, the case representation $\mathbf{x}$ should be agnostic to entities mentioned in $q$.
Therefore, we replace all tokens of entity mentions in $q$ with a special $\texttt{<MASK>}$ token from the language model.

Next, a set of inferential chains $\mathcal{P}$ is derived from the question $q$ and the answer set $\mathcal{E}_a$.
From the question $q$, a set of query entities $\mathcal{E}_q$ is extracted, forming a set of source nodes of reasoning chains over the knowledge base $K$.
In practice, this step is accomplished by detecting the entity mentioned in $q$ and performing entity linking to the knowledge base $K$.
Since our focus is on the reasoning step, we follow the same experiment setup of [?] and assume that $\mathcal{E}_q$ is also given.
Given the set of query entities $e_q (e_q\in \mathcal{E}_q)$ and the set of answer entities $e_a (e_a\in \mathcal{E}_a)$, we find all the paths between them in $K$.
Formally, let $p$ be the shortest path from $e_q$ to $e_a$ in $K$, denoting $p\colon e_q \xrightarrow{r_i} e_i  \xrightarrow{r_j}... \xrightarrow{r_n} e_a$, where $r_i, r_j,... \in R$ are the relation edges. 
% \td{
% Formally, we denote the shortest path $p$ from $e_q$ to $e_a$ in $K$ as $e_q \xrightarrow{r_i} e_i  \xrightarrow{r_j}\dots\xrightarrow{r_n} e_a$, where $r_i,\dots,r_n$ are relation edges. }
% \td{Note: using $\dots$ instead of ...}
The corresponding inferential chain $\mathbf{p} \in \mathcal{P}$ is an ordered list $[r_i ... r_n]$ extracted from $p$, where $n$ is the number of hops to reach the answer from the question.
% In summary, each case $c$ in the case-base $\mathcal{C}$ is defined as:
% $$
% c \coloneqq (\mathbf{x}, \mathcal{P}) \coloneqq \big(\texttt{LM}(q_{\texttt{<MASK>}}), \{\mathbf{p} \mid K, \mathcal{E}_q, \mathcal{E}_a \}\big)
% $$
% \td{We may want to move this definition to the top as we are likely to explain them}

\subsection{Retrieving Similar Cases}
\label{subsec:similarity}
Given a new target question $q_{\texttt{tgt}}$, the first step of our proposed CBR system is retrieving similar cases $c_{\texttt{knn}}$ from the case-base $\mathcal{C}$.
To do so, we employ the dense-retriever $\texttt{FAISS}$~\cite{faiss} and populate its index with vectors of case representations in $\mathcal{C}$. {\color{red}Should we actually mention how such vectors are created? what embeddings ... etc}
We form the query $\mathbf{x}_{\texttt{tgt}}$ for the dense-retriever by encoding the target question using the same procedure and pretrained language model as we did for questions in the case-base.
The dense-retriever provides a similarity ranking between the target question embedding $\textbf{x}_{\texttt{tgt}}$ and all cases in $\mathcal{C}$ based on the cosine-similarity of their embeddings.
We gather cases with the top-k scores from this ranking\footnote{If there are cases with the same score then all of them will be included.}, and for each k-nearest neighbor (k-NN) case ($c_{\texttt{knn}}$), we collect its corresponding set of inferential chains or inferential set $\mathcal{P}$ in short.
At the end of the CBR retrieve step, we obtain a collection $\{\mathcal{P}_i\}_{i=1}^k$ of the inferential sets of k-NN cases.

\subsection{Reusing Inferential Chains}
The CBR hypothesis [?] states that similar problems should have similar solutions.
In our scenario, correct inferential chains of the target question should be similar to retrieved inferential chains.
One might even think that traversing the knowledge base using the same steps in retrieved inferential chains would yield desired answers.
Indeed, it is possible to obtain answers this way if the knowledge base is complete or ideal, i.e., the KB covers all world facts.
However, in practice, the KB is often sparse which results in different inferential chains for the same semantic behavior ({\color{red}see Figure [?]}).
Hence, we propose an algorithm for reusing retrieved inferential chains that are robust to the sparsity or incompleteness of knowledge bases.
{\color{red}An overview of our proposed algorithm is depicted in Algorithm [?].}

We propose a majority voting scheme where each k-NN case casts a voting score for each candidate answering node, based on its set of inferential chains.
Voting scores are aggregated across cases, and candidate nodes with the highest scores are returned as predicted answers.
Intuitively, \method{} scans all possible k-NN solutions, applies them to solve the target question, and picks answers that have high scores and appear frequently enough (the most reliable answers).

Next, we describe how \method{} computes voting scores from its inferential set $\mathcal{P}$.
Consider the target question $q_{\texttt{tgt}}$, we obtain its set of query entities $\mathcal{E}_0$, and its candidate sub-KB $K_{\texttt{tgt}}$ similar to [?]. 
For each inferential chain $\mathbf{p}_{\texttt{knn}} \in \mathcal{P}$, we propose a beam search procedure that softly-following $\mathbf{p}_{\texttt{knn}}$’s relation edges on $K_{\texttt{tgt}}$. Specifically, starting from $e_0 \in \mathcal{E}_0$ and $r_0 \in \mathbf{p}_{\texttt{knn}}$, the beam search step finds a \textit{plausible} relation edge $\hat{r_0} \in K_{\texttt{tgt}}$ that matches $r_0$ and follows $\hat{r_0}$ to reach some entity nodes $e_1 \in \mathcal{E}_1$.
This beam search step is repeated for the rest of relation edge $r_i \in \mathbf{p}_{\texttt{knn}}$ in their corresponding order.
For each beam search step, a score of how likely the \textit{plausible} relation $\hat{r_i}$ holds in $K_{\texttt{tgt}}$ is also computed.
At the end of the beam search procedure, all entities in $\mathcal{E}_n$ are assigned the beam search score as their voted scores.

We employ several methods for finding the \textit{plausible} relation $\hat{r_i} \in K_{\texttt{tgt}}$, depends on $r_i \in \mathbf{p}_{\texttt{knn}}$ and the target knowledge graph $K_{\texttt{tgt}}$.
Recall that by our definition of the knowledge base in Section [2], $r_i$ can be a symbolic relation predefined by the KB, or it can be a free-form relation indicated by a short-text document.
In case $r_i$ is a symbolic relation, or formally $r_i \in R$, \method{} forms a structure query $(e_i, r_i, ?)$ \textit{over the full knowledge base} $K$.
To execute this query, we use both exact matching of $r_i$, and a pre-trained knowledge base completion model [?], namely $\texttt{KBC}$.
Here we note that this query is executed over the full KB instead of the target sub-KB $K_{\texttt{tgt}}$, allowing \method{} to consider all possible entities in the KB.

In addition, we utilize the set of free-form relations $d \in D$ that stem from $e_i$, checking whether they serve as evidence for how likely $r_i$ holds between $e_i$ and other entities mentioned in $d$.  
For this purpose, we employ an off-the-shelve relation extraction model $\texttt{RE}$ [?] specifically chosen for each benchmark ({\color{red}see details in Section [?]}).
Typically, a relation extraction model predicts a relation label for an entity pair mentioned in the given text, and the set of relation labels might not be aligned with $R$.
To avoid this relation set mismatch, we suggest using a fixed proxy-text $d_{r_i}$ for all relation $r_i \in R$.
A symbolic relation $r_i \in R$ is said to be supported by the document $d \in D$ if the relation extraction model $\texttt{RE}$ predicts to the same relation given $d_{r_i}$and given $d$.
In summary, for a symbolic relation $r_i \in \mathbf{p}_{\texttt{knn}}$ and $r_i \in R$, $r_i$ plausibly holds for $e_i$ and some entities $e_{i+1} \in \mathcal{E}_{i+1}$with some score $s_i$ defined as follow:
$$
s_i \coloneqq 
\begin{cases}
1.0 & \text{if } (e_i, r_i, e_{i+1}) \in K\\
\texttt{KBC}(e_i, r_i, e_{i+1}) &\\
\text{Pr}\big(\texttt{RE}(d_{r_i}) = \texttt{RE}(d)) & \text{if } (e_i, d, e_{i+1}) \in K
\end{cases}
$$
When $r_i$ a free-form relation indicated by the document $d \in D$, we align it to a relation $r_j \in R$ using the relation extraction model. More specifically, 
$$
r_j \coloneqq \argmax_{\forall r_k \in R}{ \text{ Pr} (\texttt{RE}(d) = \texttt{RE}(d_{r_k}))}
$$
We next use $r_j$ as the plausible relation to follow from $e_i$, similar as previously described.
The scores for all entities $e_{i+1}$ resulting from following $r_j$ from $e_i$ now become:
$$
s_i \coloneqq \text{ Pr} (\texttt{RE}(d) = \texttt{RE}(d_{r_j})) * s_j
$$
where $s_j$ is computed for $r_j$ with Equation [?].

\subsection{Revising and Retaining Solutions}
So far, we assume that inferential chains obtained from k-nearest neighbor cases are equally correct. 
However, inferential chains are inferred from question-answers pairs and sometimes are spurious as briefly discussed in Section [?].
To alleviate the effect of spurious chains, we introduce a CBR revise step that utilizes a cross-validation set to provide a ranking over inferential chains.
Inferential chains with higher ranks are retained in the case-base.
Meanwhile, low-ranked chains with scores below a thresh-hold are considered spurious and are discarded from the case-base.

Our revise step is based on three main observations.
First, if a question has multiple answers, inferential chains should be consistent across all answers.
{\color{red}For instance, in Figure [?] the inferential chain $[...]$ can be derived for the answer `xxx', however it is not applicable to answer `yyy'.}
Here, one can see that spurious inferential chains might result in false negatives.
On the other hand, a correct inferential chain might as well introduce false negatives due to missing KB relations as shown in Figure [?].
Therefore we cannot immediately discard inferential chains with false negatives. 
Still we can claim that the less false negatives, the more reliable inferential chains are.

After extracting inferential chains from reasoning chains, we can execute inferential chains on the knowledge base.
If inferential chains are spurious, they sometimes introduce additional answers (see Figure [?]).
Ideally, this property is unique to spurious chains as correct inferential chains are bound to only correct answers.
However, in practice some correct answers might be missing from the gold answer set due to annotation errors.
These missing answers might become false positives even for correct inferential chains.
Again, false positives are not explicit indicators that inferential chains are spurious, but they are useful indicators how precise inferential chains are.

Recall the CBR hypothesis that similar problems should have similar solutions, the two mentioned properties should hold not only for the question which inferential chains are derived from, but also for similar questions.
Combining the three observations, we suggest that the F1 scores [?] are computed for inferential chains in the case-base over (1) corresponding questions they are derived from and (2) similar questions from a cross-validation set.
While the first set of F1 scores tells us how locally consistent inferential chains are, the second set of F1 scores lets us know how they are globally consistent with similar examples.
We rank inferential chains based on the first then the second F1 scores, and retain only top inferential chains.

==> notation.tex <==
\newcommand{\cbrsup}{\textsc{Cbr-kbqa}\xspace}

==> related_work.tex <==
\section{Related Work}
\td{\textbf{Weak-Supervised KBQA.} Survey GRAFT-Net, PullNet, ReTraCk, ReifKB, LEGO, EmQL, EmbedKGQA, KAR, STAGG, QGG. State the gap with supervised methods RNG-KBQA, CBR-KBQA}.

\noindent\td{\textbf{QA over Incomplete KB.} Survey methods using text. Survey method using pre-trained KBC}

==> table.tex <==
\begin{table*}[t]
    \caption{\textbf{AAA.}} 
    
    \centering
        \begin{tabular}{l|ccc|c|c}
        \hline Model & \multicolumn{3}{|c|}{ MetaQA } & \multirow{2}{*}{ WebQSP } & \multirow{2}{*}{ CompWebQ } \\
        \cline { 2 - 4 } & 1-hop & 2-hop & 3-hop & & \\
        \hline KVMemNN (Miller et al., 2016) & $95.8$ & $25.1$ & $10.1$ & $46.7$ & $21.1$ \\
        VRN (Zhang et al., 2017) & $\mathbf{9 7 . 5}$ & $89.9$ & $62.5$ & $-$ & $-$ \\
        GraftNet (Sun et al., 2018) & $97.0$ & $94.8$ & $77.7$ & $66.4$ & $32.8$ \\
        PullNet (Sun et al., 2019) & $97.0$ & $99.9$ & $91.4$ & $68.1$ & $47.2$ \\
        SRN (Qiu et al., 2020) & $97.0$ & $95.1$ & $75.2$ & $-$ & $-$ \\
        ReifKB (Cohen et al., 2020) & $96.2$ & $81.1$ & $72.3$ & $52.7$ & $-$ \\
        EmbedKGQA (Saxena et al., 2020) & $\mathbf{9 7 . 5}$ & $98.8$ & $94.8$ & $66.6$ & $-$ \\
        TransferNet (Shi et al., 2021) & $\mathbf{97. 5}$ & $\mathbf{1 0 0}$ & $\mathbf{1 0 0}$ & $\mathbf{7 1 . 4}$ & $\mathbf{4 8 . 6}$ \\
        \hline
        CBR-iKB (Ours) & $\mathbf{100}$ & $\mathbf{100}$ & $\mathbf{100}$ & $\mathbf{69}$ & $-$ \\
        \end{tabular}
\end{table*}
    
